Neural Natural Language Processing for Unstructured Data in Electronic Health Records: a Review

Electronic health records (EHRs), digital collections of patient healthcare events and observations, are ubiquitous in medicine and critical to healthcare delivery, operations, and research. Despite this central role, EHRs are notoriously difficult to process automatically. Well over half of the information stored within EHRs is in the form of unstructured text (e.g. provider notes, operation reports) and remains largely untapped for secondary use. Recently, however, newer neural network and deep learning approaches to Natural Language Processing (NLP) have made considerable advances, outperforming traditional statistical and rule-based systems on a variety of tasks. In this survey paper, we summarize current neural NLP methods for EHR applications. We focus on a broad scope of tasks, namely, classification and prediction, word embeddings, extraction, generation, and other topics such as question answering, phenotyping, knowledge graphs, medical dialogue, multilinguality, interpretability, etc.

==> 7_resources.tex <==
\section{Datasets and Tools}


\subsection{Datasets}

\subsubsection{General Datasets} 
   \hfill \break

  \begin{tabularx}
  {\textwidth}{|p{2cm}|p{3cm}|X|}
  \hline
  \textbf{Dataset} & \textbf{Link} & \textbf{Description} \\
  \hline
  MIMIC-III & \url{https://mimic.physionet.org/} & A free, publicly accessible database of de-identified medical information on patient stays in the critical care units of the Beth Israel Deaconess Medical Center between 2001 and 2012. The table NOTEEVENTS contains clinical notes from over 40,000 patients. Other tables have data on mortality, imaging reports, demographics, vital signs, lab tests, drugs, and procedures. MIMIC-III follows two earlier versions of MIMIC, also very popular with biomedical NLP researchers. \\ \hline
  MIMIC-CXR & \url{https://physionet.org/content/mimic-cxr/2.0.0/} & Like MIMIC-III, MIMIC-CXR contains de-identified clinical information from the Beth Israel Deaconess Medical Center. It has over 377,000 radiology images of chest X-rays. The creators of the dataset also used the ChexPert\cite{irvin2019chexpert} tool to classify each image's corresponding free-text note into 14 different labels. \\ \hline
  NUBes-PHI & N/A &  A Spanish medical report corpus, containing about 7,000 real reports with annotated negation and uncertainty information \cite{lima2020nubes}. \\ \hline
  Abbrev dataset & \url{https://nlp.cs.vcu.edu/data.html} & This dataset is a re-creation of an old dataset which contains the acronyms and long-forms from Medline abstracts. It is automatically re-created by identifying the acronyms long forms in the Medline abstract and replacing it with it's acronym. There are three subsets containing 100, 200 and 300 instances respectively. \\ \hline 
  MEDLINE & \url{ https://www.nlm.nih.gov/bsd/medline.html} & A database of 26 million journal articles on biomedicine and health from 1950 to the present. It is compiled by the United States National Library of Medicine (NLM). \\ \hline
  MedlinePlus & \url{ https://www.nlm.nih.gov/bsd/medline.html} & Related to MEDLINE, it describes medical terms in simple language. \\ \hline
  PubMed & \url{ https://www.ncbi.nlm.nih.gov/guide/howto/obtain-full-text/} & A corpus containing more than 30 million citations for biomedical and scientific literature. In addition to MEDLINE, these texts come from sources like online books, papers on other scientific topics, and biomedical articles that have not been processed by MEDLINE. \\ \hline
\end{tabularx}



% \textbf{MIMIC-III}\footnote{\url{https://mimic.physionet.org/}} 
% A free, publicly accessible database of de-identified medical information on patient stays in the critical care units of the Beth Israel Deaconess Medical Center between 2001 and 2012. The table NOTEVENTS contains clinical notes from over 40,000 patients. Other tables have data on mortality, imaging reports, demographics, vital signs, lab tests, drugs, and procedures. Before MIMIC-III, there were two other iterations of MIMIC used by biomedical NLP researchers.

% \textbf{MIMIC-CXR}\footnote{\url{https://physionet.org/content/mimic-cxr/2.0.0/}} 
% Like MIMIC-III, MIMIC-CXR contains de-identified clinical information from the Beth Israel Deaconess Medical Center. It has over 377,000 radiology images of chest X-rays. The creators of the dataset also used the ChexPert\cite{irvin2019chexpert} tool to classify each image's corresponding free-text note into 14 different labels.

% \textbf{NUBes-PHI} \cite{lima2020nubes} A Spanish medical report corpus, containing about 7,000 real reports with annotated negation and uncertainty information.

% % \subsection{Journal Articles}

% \textbf{Abbrev dataset}\footnote{\url{https://nlp.cs.vcu.edu/data.html}} This dataset is a re-creation of an old dataset which contains the acronyms and long-forms from Medline abstracts. It is automatically re-created by identifying the acronyms long forms in the Medline abstract and replacing it with it's acronym. There are three subsets containing 100, 200 and 300 instances respectively. \cite{stevenson2009disambiguation}

% \textbf{MEDLINE}\footnote{\url{ https://www.nlm.nih.gov/bsd/medline.html}}
% A database of 26 million journal articles on biomedicine and health from 1950 to the present. It is compiled by the United States National Library of Medicine (NLM). MedlinePlus\footnote{\url{ https://www.nlm.nih.gov/bsd/medline.html}}, a related service, describes medical terms in simple language.

% \textbf{PubMed}\footnote{\url{ https://www.ncbi.nlm.nih.gov/guide/howto/obtain-full-text/}} 
% A corpus containing more than 30 million citations for biomedical and scientific literature. In addition to MEDLINE, these texts come from sources like online books, papers on other scientific topics, and biomedical articles that have not been processed by MEDLINE. 


\subsubsection{Task-Specific Datasets}

   \hfill \break

  \begin{tabularx}{\textwidth}{|p{2cm}|p{3cm}|X|}
  \hline
  \textbf{Dataset} & \textbf{Link} & \textbf{Description} \\
  \hline
  BioASQ & \url{ http://bioasq.org/} & An organization that designs challenges for biomedical NLP tasks. While BioASQ challenges focus primarily on question answering (QA) and semantic indexing, some use other tasks including multi-document summarization, information retrieval, and hierarchical text classification. \\ \hline
  BIOSSES & \url{http://tabilab.cmpe.boun.edu.tr/BIOSSES/} & A benchmark dataset for biomedical sentence similarity estimation \cite{souganciouglu2017biosses}. \\ \hline 
  BLUE & \url{https://github.com/ncbi-nlp/BLUE_Benchmark} & Biomedical Language Understanding Evaluation (BLUE) is a collection of ten datasets for five biomedical NLP tasks. These tasks cover sentence similarity, named entity recognition, relation extraction, document classification, and natural language inference. BLUE serves as a useful benchmarking tool, as it centralizes the datasets that medical NLP systems evaluate on. \\ \hline 
  Clinical Abbreviation Sense Inventory & \url{https://conservancy.umn.edu/handle/11299/137703} & A dataset for medical term disambiguation. In the latest version, 440 of the most frequently used abbreviations and acronyms were selected from 352,267 dictated clinical notes. \\ \hline
  CLINIQPARA & N/A & A dataset with paraphrases for clinical questions. Contains 10,578 unique questions across 946 semantically distinct paraphrase clusters. Initially collected for improving question answering for EHRs. \\ \hline
  i2b2 & \url{ http://www.i2b2.org/} & Informatics for Integrating Biology and the Bedside, or i2b2, is a non-profit that organizes datasets and competitions for clinical NLP. It has numerous datasets for specific tasks like deidentification, relation extraction, clinical trial cohort selection. These datasets and challenges are now run by Harvard's National NLP Clinical Challenges, or n2c2; however, most papers refer to them with the name i2b2. \\ \hline 
  MedICaT & \url{ https://github.com/allenai/medicat} & A collection of more than 217,000 medical images, corresponding captions, and inline references, made for figure retrieval and figure-to-text alignment tasks. Unlike previous medical imaging datasets, subfigures and subcaptions are explicitly aligned, introducing the specific task of subcaption-subfigure alignment. \\ \hline 
  MedNLI & \url{ https://jgc128.github.io/mednli/} & Designed for Natural Language Inference (NLI) in the clinical domain. The objective of NLI is to predict whether a hypothesis can be deemed true, false, or undetermined from a given premise. MedNLI contains 14,049 unique sentence pairs, annotated by 4 clinicians over the course of six weeks. To download it, one first needs to get access to MIMIC-III. \\ \hline 
  MedQuAD & \url{https://github.com/abachaa/MedQuAD} & Medical Question Answering Dataset, a collection of 47,457 medical question-answer pairs created from 12 NIH websites (e.g. cancer.gov, niddk.nih.gov, GARD, MedlinePlus Health Topics). There are 37 question types associated with diseases, drugs and other medical entities such as tests
  \cite{019arXiv190108079A}. \\ \hline 
\end{tabularx}
\newpage
\begin{tabularx}{\textwidth}{|p{2cm}|p{3cm}|X|}
  \hline
  VQA-RAD & \url{https://osf.io/89kps/} & A dataset of manually constructed question-answer pairs corresponding to radiology images. It was designed for future Visual Question Answering systems, which will automatically answer salient questions on X-rays. These models will hopefully be very useful clinical decision support tools for radiologists. \\ \hline 
  WikiMed and PubMedDS & N/A &  Two large-scale datasets for entity linking \cite{vashishth2020medtype}. WikiMed contains over includes 650,000 mentions normalized to concepts in UMLS. PubMedDS is an annotated corpus with more than 5 million normalized mentions spanning across 3.5 million documents. \\ \hline
  PathVQA & N/A & The first dataset for pathology visual question answering \cite{he2020pathvqa}. It contains manually-checked 32,799 questions from 4,998 pathology images. \\ \hline 
  MedQA & N/A & \cite{jin2020disease} The first multiple-choice OpenQA dataset
for solving medical problems. The dataset is collected from professional medical board exams in three languages: English, simplified Chinese, and traditional Chinese, with 12,723, 34,251, and 14,123 questions respectively. \\ \hline
\end{tabularx}

% \textbf{BioASQ}\footnote{\url{ http://bioasq.org/}} 
% An organization that designs challenges for biomedical NLP tasks. While BioASQ challenges focus primarily on question answering (QA) and semantic indexing, some use other tasks including multi-document summarization, information retrieval, and hierarchical text classification.


% \textbf{BIOSSES} \footnote{\url{http://tabilab.cmpe.boun.edu.tr/BIOSSES/}} \cite{souganciouglu2017biosses} A benchmark dataset for biomedical sentence similarity estimation. 


% \textbf{BLUE} \footnote{\url{https://github.com/ncbi-nlp/BLUE_Benchmark}} 
% Biomedical Language Understanding Evaluation (BLUE) is a collection of ten datasets for five biomedical NLP tasks. These tasks cover sentence similarity, named entity recognition, relation extraction, document classification, and natural language inference. BLUE serves as a useful benchmarking tool, as it centralizes the datasets that medical NLP systems evaluate on.

% \textbf{Clinical Abbreviation Sense Inventory}\footnote{\url{https://conservancy.umn.edu/handle/11299/137703}}
% A dataset for medical term disambiguation. In the latest version, 440 of the most frequently used abbreviations and acronyms were selected from 352,267 dictated clinical notes.

% \textbf{CLINIQPARA}\cite{soni2019paraphrase} A dataset with paraphrases for clinical questions. Contains 10,578 unique questions across 946 semantically distinct paraphrase clusters. Initially collected for improving question answering for EHRs.


% \textbf{i2b2}\footnote{\url{ http://www.i2b2.org/}} 
% Informatics for Integrating Biology and the Bedside, or i2b2, is a non-profit that organizes datasets and competitions for clinical NLP. It has numerous datasets for specific tasks like deidentification, relation extraction, clinical trial cohort selection. These datasets and challenges are now run by Harvard's National NLP Clinical Challenges, or n2c2; however, most papers refer to them with the name i2b2.

% \textbf{MedICaT}\footnote{\url{ https://github.com/allenai/medicat}}
% A collection of more than 217,000 medical images, corresponding captions, and inline references, made for figure retrieval and figure-to-text alignment tasks. Unlike previous medical imaging datasets, subfigures and subcaptions are explicitly aligned, introducing the specific task of subcaption-subfigure alignment.

% \textbf{MedNLI}\footnote{\url{ https://jgc128.github.io/mednli/}} 
% Designed for Natural Language Inference (NLI) in the clinical domain. The objective of NLI is to predict whether a hypothesis can be deemed true, false, or undetermined from a given premise. MedNLI contains 14,049 unique sentence pairs, annotated by 4 clinicians over the course of six weeks. To download it, one first needs to get access to MIMIC-III.

% \textbf{MedQuAD}\footnote{\url{https://github.com/abachaa/MedQuAD}}
% Medical Question Answering Dataset, a collection of 47,457 medical question-answer pairs created from 12 NIH websites (e.g. cancer.gov, niddk.nih.gov, GARD, MedlinePlus Health Topics). There are 37 question types associated with diseases, drugs and other medical entities such as tests. \cite{019arXiv190108079A}

% \textbf{VQA-RAD}\footnote{\url{https://osf.io/89kps/}} 
% A dataset of manually constructed question-answer pairs corresponding to radiology images. It was designed for future Visual Question Answering systems, which will automatically answer salient questions on X-rays. These models will hopefully be very useful clinical decision support tools for radiologists.

% \textbf{WikiMed and PubMedDS} \cite{vashishth2020medtype} Two large-scale datasets for entity linking. WikiMed contains over includes 650,000 mentions normalized to concepts in UMLS. PubMedDS is an annotated corpus with more than 5 million normalized mentions spanning across 3.5 million documents. 


% \textbf{PathVQA}
% \cite{he2020pathvqa} The first dataset for pathology visual question answering. It contains manually-checked 32,799 questions from 4,998 pathology images.

% \textbf{MedQA}
% \cite{jin2020disease} The first multiple-choice OpenQA dataset
% for solving medical problems. The dataset is collected from professional medical board exams on three languages: English, simplified Chinese, and traditional Chinese. For the languages, there are 12,723, 34,251, and 14,123 questions respectively. 

\subsection{Tools and libraries}


\subsubsection{Machine Learning}

   \hfill \break

  \begin{tabularx}{\textwidth}{|p{2cm}|p{3cm}|X|}
  \hline
  \textbf{Tool} & \textbf{Link} & \textbf{Description} \\
  \hline
  Pytorch & \url{ https://pytorch.org/} & Pytorch is an open source deep learning library developed by Facebook, primarily for use in Python. It is a leading platform in both industry and academia. \\ \hline 
  Scikit-learn & \url{https://scikit-learn.org/} & An open python library providing efficient data mining and data analysis tools. These includes methods for classification, regression, clustering, etc. \\ \hline 
  TensorFlow & \url{https://www.tensorflow.org/} & Google's open-source framework for efficient computation, used primarily for machine learning. Tensorflow provides stable APIs for Python and C; it has also been adapted for use in a variety of other programming languages.\\ \hline
  \end{tabularx}
  
% \textbf{Pytorch} \footnote{\url{ https://pytorch.org/}}
% Pytorch is an open source deep learning library developed by Facebook, primarily for use in Python. It is a leading platform in both industry and academia.

% \textbf{Scikit-learn}\footnote{\url{https://scikit-learn.org/}}
% An open python library providing efficient data mining and data analysis tools. These includes methods for classification, regression, clustering, etc. 

% \textbf{TensorFlow}\footnote{\url{https://www.tensorflow.org/}} Google's open-source framework for efficient computation, used primarily for machine learning. 
% %In general, TensorFlow is more popular than Pytorch in industry, whereas in academe Pytorch is more common. 
% Tensorflow provides stable APIs for Python and C; it has also been adapted for use in a variety of other programming languages.

\subsubsection{NLP}

\hfill \break

\begin{tabularx}{\textwidth}{|p{2cm}|p{3cm}|X|}
  \hline
  \textbf{Tool} & \textbf{Link} & \textbf{Description} \\
  \hline
  AllenNLP & \url{https://allennlp.org/} & An open-source NLP research library built on PyTorch. AllenNLP has a number of state-of-the-art models readily available, making it very easy for anyone to use deep learning on NLP tasks. \\ \hline 
  Fairseq & \url{https://github.com/pytorch/fairseq} & A Python toolkit for sequence modeling. It enables users to train custom models for text generation tasks like machine translation, summarization, and language modeling. \\ \hline 
  FastText & \url{https://fasttext.cc/} & A sequence modeling toolkit which allows users to train custom models for translation, summarization, language modeling and other text generation tasks. \\ \hline
  Gensim & \url{https://radimrehurek.com/gensim/index.html} & A scalable, robust, efficient and hassle-free python library for unsupervised semantic modelling from plain text. It has a wide range of tools for topic modeling, document indexing, and similarity retrieval. \\ \hline
  Natural Language Toolkit (NLTK) & \url{https://www.nltk.org/} & A leading platform for building Python programs concerned with human language data. It contains helpful functions for tasks such as tokenization, cleaning, and topic modeling. \\ \hline 
  PyText & \url{https://pytext-pytext.readthedocs-hosted.com/en/latest/} & PyText is a deep-learning based NLP modeling framework built on PyTorch, providing pre-trained models for NLP tasks such as sequence tagging, classification, and contextual intent-slot models. \\ \hline
  SpaCy & \url{https://spacy.io/} & A remarkably fast Python library for modeling and processing text in 34 different languages. It includes pretrained models to predict named entities, part-of-speech tags and syntactic dependencies, as well as starter models designed for transfer learning. It also has tools for tokenization, text cleaning, and statistical modeling. \\ \hline 
  Stanford CoreNLP & \url{https://stanfordnlp.github.io/CoreNLP/} & A set of tools developed by Stanford NLP Group for statistical, neural, and rule-based problems in computational linguistics. Its software provides a simple, useful interface for NLP tasks like NER and part-of-speech (POS) tagging. \\ \hline
  \end{tabularx}
  
% \textbf{AllenNLP}\footnote{\url{https://allennlp.org/}} An open-source NLP research library built on PyTorch. AllenNLP has a number of state-of-the-art models readily available, making it very easy for anyone to use deep learning on NLP tasks.
	
% \textbf{Fairseq}\footnote{\url{https://github.com/pytorch/fairseq}} A Python toolkit for sequence modeling. It enables users to train custom models for text generation tasks like machine translation, summarization, and language modeling.
	
% \textbf{FastText}\footnote{\url{https://fasttext.cc/}} A sequence modeling toolkit which allows users to train custom models for translation, summarization, language modeling and other text generation tasks.

% \textbf{Gensim}\footnote{\url{https://radimrehurek.com/gensim/index.html}} A scalable, robust, efficient and hassle-free python library for unsupervised semantic modelling from plain text. It has a wide range of tools for topic modeling, document indexing, and similarity retrieval.

% \textbf{Natural Language Toolkit (NLTK)}\footnote{\url{https://www.nltk.org/}} A leading platform for building Python programs concerned with human language data. It contains helpful functions for tasks such as tokenization, cleaning, and topic modeling. 

% \textbf{PyText} \footnote{\url{https://pytext-pytext.readthedocs-hosted.com/en/latest/}}  PyText is a deep-learning based NLP modeling framework built on PyTorch, providing pre-trained models for NLP tasks such as sequence tagging, classification, and contextual intent-slot models.

% \textbf{SpaCy}\footnote{\url{https://spacy.io/}} A remarkably fast Python library for modeling and processing text in 34 different languages. It includes pretrained models to predict named entities, part-of-speech tags and syntactic dependencies, as well as starter models designed for transfer learning. It also has tools for tokenization, text cleaning, and statistical modeling.

% \textbf{Stanford CoreNLP}\footnote{\url{https://stanfordnlp.github.io/CoreNLP/}} A set of tools developed by Stanford NLP Group for statistical, neural, and rule-based problems in computational linguistics. Its software provides a simple, useful interface for NLP tasks like NER and part-of-speech (POS) tagging. 


\subsubsection{Clinical NLP}

\hfill \break

\begin{tabularx}{\textwidth}{|p{2cm}|p{3cm}|X|}
  \hline
  \textbf{Tool} & \textbf{Link} & \textbf{Description} \\
  \hline
  Criteria2Query & \url{http://www.ohdsi.org/web/criteria2query/} & A system for automatically transforming clinical research eligibility criteria to Observational Medical Outcomes Partnership (OMOP) Common Data Model-based executable cohort queries. \cite{yuan2019criteria2query} The system is an information extraction pipeline that combines machine learning and rule-based methods. \\ \hline 
  CuiTools & \url{http://cuitools.sourceforge.net/} & A package of PERL programs for word sense disambiguation (WSD)\cite{mcinnes2007using}. Its models perform supervised or unsupervised WSD using both general English knowledge and specific medical concepts extracted from UMLS. \\ \hline
  Metamap & \url{https://metamap.nlm.nih.gov/} & A tool to identify medical concepts from the text and map them to standard terminologies in the UMLS. MetaMap uses a knowledge-intensive approach based on symbolic, NLP and computational-linguistic techniques. \\ \hline 
  MIMIC-Extract & \url{https://github.com/MLforHealth/MIMIC_Extract} & An open source pipeline to preprocess and present data from MIMIC-III v1.4 database. \cite{wang2020mimic} MIMIC-Extract has useful features for analysis - for example, it transforms discrete temporal data into a time-series, and extracts clinically relevant targets like mortality from the text. \\ \hline
  ScispaCy & \url{https://allenai.github.io/scispacy/} &  Many NLP models perform poorly under domain shift, so ScispaCy adapts SpaCy's models to process scientific, biomedical, or clinical text. It was developed by AllenNLP in 2019 and includes much of the same functionality as SpaCy. \\ \hline
  Unified Medical Language System (UMLS) & \url{https://www.nlm.nih.gov/research/umls/} & UMLS is a set of files and software that provides unifying relationships across a number of different medical vocabularies and standards. Its aim is to improve effectiveness and interoperability between biomedical information systems like EHRs. It can be used to link medical terms, drug names, or billing codes across different computer systems. \\ \hline 
\end{tabularx}

% \textbf{Criteria2Query} \footnote{\url{http://www.ohdsi.org/web/criteria2query/}} A system for automatically transforming clinical research eligibility criteria to Observational Medical Outcomes Partnership (OMOP) Common Data Model-based executable cohort queries. \cite{yuan2019criteria2query} The system is an information extraction pipeline that combines machine learning and rule-based methods. 

% \textbf{CuiTools} \footnote{\url{http://cuitools.sourceforge.net/}}
%  A package of PERL programs for word sense disambiguation (WSD)\cite{mcinnes2007using}. Its models perform supervised or unsupervised WSD using both general English knowledge and specific medical concepts extracted from UMLS.
 
% \textbf{Metamap}\footnote{\url{https://metamap.nlm.nih.gov/}} A tool to identify medical concepts from the text and map them to standard terminologies in the UMLS. MetaMap uses a knowledge-intensive approach based on symbolic, NLP and computational-linguistic techniques.

% \textbf{MIMIC-Extract} \footnote{\url{https://github.com/MLforHealth/MIMIC_Extract}} An open source pipeline to preprocess and present data from MIMIC-III v1.4 database. \cite{wang2020mimic} MIMIC-Extract has useful features for analysis - for example, it transforms discrete temporal data into a time-series, and extracts clinically relevant targets like mortality from the text.

% \textbf{ScispaCy}\footnote{\url{https://allenai.github.io/scispacy/}} Many NLP models perform poorly under domain shift, so ScispaCy adapts SpaCy's models to process scientific, biomedical, or clinical text. It was developed by AllenNLP in 2019 and includes much of the same functionality as SpaCy.

% \textbf{Unified Medical Language System (UMLS)}\footnote{\url{https://www.nlm.nih.gov/research/umls/}} UMLS is a set of files and software that provides unifying relationships across a number of different medical vocabularies and standards. Its aim is to improve effectiveness and interoperability between biomedical information systems like EHRs. It can be used to link medical terms, drug names, or billing codes across different computer systems. 	


